An Analysis of Speculative Type Confusion Vulnerabilities in the Wild

Spectre v1 attacks, which exploit conditional branch misprediction, are often identified with attacks that bypass array bounds checking to leak data from a victim's memory. Generally, however, Spectre v1 attacks can exploit any conditional branch misprediction that makes the victim execute code incorrectly. In this paper, we investigate speculative type confusion, a Spectre v1 attack vector in which branch mispredictions make the victim execute with variables holding values of the wrong type and thereby leak memory content. We observe that speculative type confusion can be inadvertently introduced by a compiler, making it extremely hard for programmers to reason about security and manually apply Spectre mitigations. We thus set out to determine the extent to which speculative type confusion affects the Linux kernel. Our analysis finds exploitable and potentially-exploitable arbitrary memory disclosure vulnerabilities. We also find many latent vulnerabilities, which could become exploitable due to innocuous system changes, such as coding style changes. Our results suggest that Spectre mitigations which rely on statically/manually identifying "bad" code patterns need to be rethought, and more comprehensive mitigations are needed.

==> ebpf-mitigation.tex <==
\section{Discussion \& mitigations} \label{sec:discussion}

\paragraph{Hardware mitigations}
The attacks would become harder to mount if user and kernel context used different BPUs.
This mitigation still allows attackers to perform mistraining (at least in principle) by invoking
shadow branches in the kernel, whose PHT entries collide with the target branch.

\paragraph{Securing eBPF}

eBPF can defend from speculative type confusion in eBPF-specific
ways.  The verifier can reason about all execution flows, not just
semantically correct ones.  However, this approach would increase verification time and render
some programs infeasible to verify.  An alternative approach is for the verifier to inject masking
instructions to ensure that the operand of \emph{every} load instruction is constrained to the object
it is supposed to be accessing, generalizing the Native Client x86-64 sandboxing approach~\cite{NACL_SFI}.

